Modeling Long Cycles

Recurrent boom-and-bust cycles are a salient feature of economic and financial history. Cycles found in the data are stochastic, often highly persistent, and span substantial fractions of the sample size. We refer to such cycles as "long". In this paper, we develop a novel approach to modeling cyclical behavior specifically designed to capture long cycles. We show that existing inferential procedures may produce misleading results in the presence of long cycles, and propose a new econometric procedure for the inference on the cycle length. Our procedure is asymptotically valid regardless of the cycle length. We apply our methodology to a set of macroeconomic and financial variables for the U.S. We find evidence of long stochastic cycles in the standard business cycle variables, as well as in credit and house prices. However, we rule out the presence of stochastic cycles in asset market data. Moreover, according to our result, financial cycles as characterized by credit and house prices tend to be twice as long as business cycles.

==> Conclusion.tex <==
% !TEX root = long_cycles_main.tex

\section{Conclusion}

This paper presents a new econometric model that captures the persistent and low-frequency oscillations in time series data. It extends the local-to-unity model by introducing another localization parameter that controls the frequency of oscillation. This additional parameter allows us to model cyclical processes where the cycle length is long relative to the sample size. Such long-cycle processes are near I(2) and have a different asymptotic distribution from the near-integrated processes. We derive the asymptotic theory for long-cycle processes and the relevant regression statistics.

Based on the new theory, we propose a uniformly valid inference procedure for testing the periodicity of cycles in data. We apply our procedure to examine the cyclical properties of key macroeconomic and financial time series in the U.S. Our empirical findings support the view of endogenous business cycles, and corroborate that financial cycles tend to be much longer than business cycles. Moreover, we find no evidence of stochastic cycles in equity prices, volatility index and credit risk premium, suggesting that risk perception and risk-bearing capacity are not what drive business cycle fluctuations. 

The theory developed in this paper also provides the foundation for inferential analysis of long-cycle data to address the questions of cointegration and phase shifts in macro-financial aggregates. These are left for future research. 





 












